RNN Architecture Learning with Sparse Regularization

Neural models for NLP typically use large numbers of parameters to reach state-of-the-art performance, which can lead to excessive memory usage and increased runtime. We present a structure learning method for learning sparse, parameter-efficient NLP models. Our method applies group lasso to rational RNNs (Peng et al., 2018), a family of models that is closely connected to weighted finite-state automata (WFSAs). We take advantage of rational RNNs' natural grouping of the weights, so the group lasso penalty directly removes WFSA states, substantially reducing the number of parameters in the model. Our experiments on a number of sentiment analysis datasets, using both GloVe and BERT embeddings, show that our approach learns neural structures which have fewer parameters without sacrificing performance relative to parameter-rich baselines. Our method also highlights the interpretable properties of rational RNNs. We show that sparsifying such models makes them easier to visualize, and we present models that rely exclusively on as few as three WFSAs after pruning more than 90% of the weights. We publicly release our code.

==> text/background.tex <==
\section{Background}
\label{sec:background}

We aim to learn parameter-efficient models using sparse regularization. 
Methods that encourage sparsity like group lasso~\citep{group_lasso} 
assume that features can be meaningfully grouped.  
Such methods were popular when applied to linear models in NLP~\citep{Martins:2011}, 
where handcrafted features were grouped by the templates they instantiated. 
In neural NLP models, parameters are typically less interpretable, 
and hence it is not straightforward how to group them~\citep{Doshi:2017}.

In this work we apply sparse regularization to rational RNNs, which allows for learning meaningful sparse structures,
 by eliminating states or transitions, and even whole WFSAs.
The main contribution of this paper is applying group lasso 
to automate choices about which states or WFSAs to eliminate, thereby learning the neural structure itself.
\resolved{\hao{i feel the above should go into method or the end of intro}\roy{I think it's fine, doesn't hurt to reiterate our story}}
We briefly review group lasso and rational RNNs.  
\resolved{\nascomment{I propose using either \lone or $\ell_1$ but really what matters here is group lasso}}

\resolved{\nascomment{I think the opening of this section needs to contextualize the roadmap. 
maybe say something like:  (1) sparsity (discussed in \S whatever) in NNs doesn't really make sense in general, but (2) it does kind of make sense of your NN is a WFSA (discussed in \S whatever), because you can think about eliminating whole states or transitions. so this paper's big contribution is to use group lasso to automate those choices about which states to eliminate, in a WFSA that's also an NN.
ALSO we shouldn't go from ``Background'' directly to ``Experiments'' -- retitle!}}


\subsection{Group Lasso Penalty}\label{sec:group_lasso}

\com{Our goal is to compress the structure of neural networks. To do so we use sparsifying regularizers, 
which learn a sparse structure of the network, and then replace the original, dense network with the smaller, sparse network.}
%We start with a brief introduction to $\ell_1$ regularization, 
%and then review group lasso. %, which we use as our sparse regularization method.
%We start by describing the $\mathbf{\ell_1}$ and lasso penalties, which motivate group lasso.

%We consider the problem of reducing the size of a neural model by removing some weights.
%When we add the $\ell_1$ norm of a parameter vector 
%(i.e., sum of absolute values of its elements) to a learner's loss function, 
%it acts as a convex, subdifferentiable approximation to the $\ell_0$ penalty,\footnote{Solving an $\ell_0$ regularized problem has been shown to be NP-Hard \cite{l0_regularization}.} known as the \textbf{lasso} \citep{lasso}\resolved{ \nascomment{add cite!}}.

This section reviews $\ell_1$ regularizer and group lasso.
When added to a learner's loss,
the $\ell_1$ norm of a parameter vector~(i.e., sum of absolute values of its elements)
acts as a convex, subdifferentiable approximation to the $\ell_0$ penalty, known as the \textbf{lasso} \citep{lasso}.\footnote{Solving an $\ell_0$ regularized problem has been shown to be NP-Hard \cite{l0_regularization}.}
% The \lone norm is formally defined as the sum of absolute values of a vector $\mathbf{v}$'s coefficients:
% \begin{equation}\label{eq:11}
% \ell_1 (\mathbf{v}) = \sum_{i} |\mathbf{v}_i|
% \end{equation}
Like the more widely used squared $\ell_2$ (``ridge'') regularizer, the lasso is used to improve generalization, usually in linear models. 
It also induces sparsity, by driving some of the parameters to zero, 
which (in the linear setting) is equivalent to eliminating 
the corresponding features. % associated with those parameters.  
Thus the lasso can promote parameter efficiency, 
and has also been argued to improve interpretability \citep{lasso}\resolved{, though there is active debate about this \citep{things} \jdcomment{these empty citations are a bit confusing to me, as i don't know what to cite here. I found a blog post by Andrew Gelman where he says the interpretability is a property of the model, not the regularization, but that doesn't seem appropriate.}}.
Like all regularizers, the lasso term is typically scaled by
a regularization strength hyperparameter (denoted by $\lambda$), 
so that the regularized learning problem is:
%While the lasso has been used to prenent overfitting and improve generalization in a similar way to the more-popular $\mathbf{\ell_2}$ regularizer, we focus on it for its ability to induce sparsity by driving weights to zero.
%This will allow us learn model strucutres that are more parameter efficient and more interpretable, as we will see.
%For a model with weights $\mathbf{w}$ and training samples $\mathbf{x}$ with labels $y$, we define $\lambda$ to be the \emph{regularization strength}, and the lasso regularized loss to be:
\begin{equation}\label{eq:1asso}
\hat{\mathbf{w}} = \argmin_\mathbf{w} \mathcal{L}(\mathbf{w}) + \lambda\sum_{i} |w_i|,
\end{equation}
%\hao{\resolved{$\mathbf{x}$ and $y$ is not introduced. and }i don't think is necessary to layout the argmin optimization problem here.}
where $\mathcal{L}$ is the training loss, and $w_i$ is a scalar parameter in the model.

{\bf Group lasso} \citep{group_lasso} generalizes the lasso to cases where a grouping of the parameters exists. 
%In group lasso, 
Here
sparsity works at the group level, driving all the parameters in a group towards zero.
Denote the parameter vector for the $g^\text{th}$ group by $\mathbf{w}_g$ (a subvector of $\mathbf{w}$).
%Let the vector of parameters for the $g^\text{th}$ group be denoted $\mathbf{w}_g$ (a subvector of $\mathbf{w}$).
The group lasso-regularized learning problem with $G$ groups is then:
\begin{equation}\label{eq:grouplasso}
\hat{\mathbf{w}} = \argmin_\mathbf{w} \mathcal{L}(\mathbf{w}) + \lambda \sum_{g=1}^{G} \sqrt{\operatorname{dim}(\mathbf{w}_g)} \norm{\mathbf{w}_g}_2,
\end{equation}
% \norm{\mathbf{w}_g}_2
with $\operatorname{dim}(\cdot)$ 
denoting the dimension of a vector.\footnote{This weighting of groups, by the square root of their sizes, is one conventional approach, but others are possible.}
% the number of parameters in $\mathbf{w}_g$.  
If every parameter is in its own group, the original lasso is recovered.

Lasso and group lasso were developed as tools for feature selection in linear models, 
but have recently been applied to neural networks~\citep{group_lasso_nn,morphnet}.
% Both are sparsifying regularizers that push parameters to zero, though their biases \hao{inductive biases?} are different. 
They are both sparsifying regularizers that push parameters to zero, with different inductive biases:  
lasso regularizes individual parameters independently, while group lasso jointly regularizes groups of parameters\com{does so wherever it lowers the objective,
while group lasso pushes groups to zero when it is helpful\roy{anything more concrete we can say here?}}.\footnote{In its simplest form, the groups do not overlap; overlapping groups are possible but require more sophisticated optimization techniques; see \citet{overlap_group_lasso} for a related discussion. Our groups are non-overlapping.}
%  \nascomment{this is just wrong; they don't specify how we optimize the function!} , and when a weight is small enough that the next gradient step would cause it to cross zero\resolved{\roy{isn't regularization strength the $\lambda$ parameter defined above?} \jdcomment{it's when the next step would make the weight cross zero, so it depends on the learning rate too}}, they set it to zero. 
%While non-group lasso would push some weights to zero, those zero weights would be spread throughout the model. 
We exploit the structure in rational RNNs for meaningful parameter grouping
(i.e., each group contains parameters associated with a WFSA state), 
so that removing a group directly shrinks a WFSA and hence the overall architecture. %neural network.

\resolved{\roy{Missing: motivation for using group lasso over lasso}}

\com{
The \lone penalty is not differentiable at zero, and thus we resort to a subgradient. 
The penalty is constant for all non-zero values, and once the parameter value is below that constant value we set it to zero (this is a threshold).  
}\resolved{\roy{Removed a couple of comments about L1, not sure whether they fit (see tex)}}

\com{
\subsubsection{justification for actually zeroing out weights}
These penalties can be viewed as a relaxation of a constrained optimization problem. \nascomment{like lasso?  I don't think this is worth talking about in this paper; better to cite past work that has effectively used structured regularizers for good benefit. Andre's EMNLP 2011 paper is a good one for NLP}
}
\subsection{WFSAs and Rational RNNs}\label{sec:wfsas}
We define a weighted finite-state automaton (WFSA) as a tuple $\langle\Sigma, \mathcal{Q}, q_0, \mathcal{F},\mathcal{T}\rangle$. $\Sigma$ is a finite alphabet, and the WFSA assigns scores to strings in $\Sigma^\ast$.  
$\mathcal{Q}$ is a finite set of states, 
$q_0 \in \mathcal{Q}$ a designated start state, 
and $\mathcal{F}\subseteq\mathcal{Q}$ is a set of final states.
$\mathcal{T}$ is a set of transitions, each a tuple of source state, target state, symbol from $\Sigma$, and weight.\footnote{Start and final states can also be weighted.
	In this work we weight them by constant 1, and suppress the definition of start and final weight functions,
	simplifying notations.
	%, simplifying notation. \resolved{\nascomment{is this correct? the old footnote just said ``we use constant 1 for both'' but didn't say whether we make some states non-initial and/or non-final, which would imply that some get weight 0.  please correct if this is wrong. I think we need to be clear here and consistent later. also,  }}
}
A path consists of a sequence of transitions, and %, and starts on an initial state and ends in a final state.
its score is computed as the product of the transition weights.
The score of an input string summarizes all the paths deriving it, either by taking the sum of all paths or the maximum-scoring path, typically calculated using dynamic programming \citep{baum_statistical_1966}.
%\com{ since the 
%transition functions are over semirings~\citep{?}}.\resolved{\roy{Dropped the last line about semirings, we don't seem to address them in this paper, might be better to stick to the forward case}}
For more discussion about WFSAs, see \citet{kuich1985semiring} .

Recently, \citet{Schwartz:2018} and
\citet{rational-recurrences} showed that several recently proposed recurrent architectures, 
including SRU \cite{Lei:2017} and quasi-RNN \cite{Bradbury:2017}, are different implementations of specific WFSAs. 
They named this family of models rational recurrent neural networks (\emph{rational RNNs}).
\footnote{\textit{Rational} follows the terminology \textit{rational power series}~\citep{berstel1988rational},the mathematical counterpart of WFSAs.}

Rational RNNs admit straightforward design of neural architectures.
For instance, the one depicted in \figref{4gram_wfsa} captures 4-gram patterns~\citep{rational-recurrences}.
%, and can be easily extended to capture, e.g., bigram patterns, by adding another state to the WFSA \cite{rational-recurrences}.
Notably, unlike traditional WFSA-based models, rational RNNs compute their WFSA scores based on word vectors (rather than word symbols), and can thus be seen as capturing ``soft'' patterns \cite{Schwartz:2018}.


An important property of rational RNNs is that, 
each WFSA state is parameterized by a separate set of parameters.
We exploit this by treating a WFSA state's parameters as a group, and applying group lasso penalty to it.
This results in dropping some states in some WFSAs (effectively making them smaller); 
those WFSAs with all of their regularized states dropped are removed entirely (effectively decreasing the RNN hidden dimension).
We then extract this sparse structure, corresponding to a version of the same RNN with far fewer parameters.
Our sentiment analysis experiments show that these thin RNNs perform on par with the original, parameter-rich RNN\resolved{, in terms of \nascomment{what}}.


\com{
	
	\figref{wfsa} presents a WFSA discussed in \citet{rational-recurrences}.
	The two transition functions $u$ and $f$ can be implemented with neural networks,
	e.g., 
	\begin{subequations}\label{eq:unigram}
		\begin{align}
		\mathbf{f}_t&=\bm{\sigma}\bigl(\mathbf{W}_{f}\mathbf{v}_{t} + \mathbf{b}_{f}\bigr),\\
		\mathbf{u}_t&=(1-\mathbf{f}_t) \odot\mathbf{W}_{u} \mathbf{v}_{t},\\
		\mathbf{c}_t &= \mathbf{f}_t\odot \mathbf{c}_{t-1}+\mathbf{u}_{t},
		\end{align}
	\end{subequations}
	where $\mathbf{v}_t$ is the word embedding vector 
	of token $x_t$ in a given input string $x_1x_2\dots x_n\in\Sigma^\ast$.
	$\{\mathbf{W}_f, \mathbf{b}_f, \mathbf{W}_u\}$ are learned parameters, and $\bm{\sigma}$ is the sigmoid function
	to act as a forget gate.
	\begin{figure}
		\centering
		\includegraphics[clip,trim=12cm 8.8cm 9cm 12cm, width=.8\columnwidth]{fig/wfsa}
		\caption{A example two-state WFSA described in \S\ref{subsec:wfsas}.}
		\label{fig:wfsa}
	\end{figure}
}


==> text/related.tex <==
\section{Related Work}


Several approaches have been proposed for reducing the size of a neural model. 
Recent advances in neural architecture search approaches have reduced the computational expense from thousands of GPU hours \cite{NAS} to tens of GPU hours \cite{efficientNAS}. 

DARTS \cite{DARTS} uses differentiable representations of neural architectures, 
and choose a compression factor before training. Then during training DARTS only keeps the K strongest connections/operations, removing the rest. While scaling K is an easy way of changing the amount of reduction in the model, their neural architecture is not learning to perform well with a subset of the parameters as ours does, it simply removes the smallest parameters. 


Our work is most similar to others which use an $\ell_1$ regularizer during training to drive parameters to zero \interalia{morphnet, group_lasso_nn,wen2016learning}, though these typically just group parameters by layers (or don't group them at all), while we take advantage of the connections between rational RNNs and WFSAs to build our groups. Alternatively, instead of using the magnitude of the parameter itself, some works have estimated the importance of a neuron with the second derivative and pruned those with small values in the Hessian \cite{brain_damage, SNIP}. 

Bayesian approaches have been used to promote sparsity by using sparsifying priors \cite{louizos2017bayesian} or using variational dropout to prune parameters \cite{molchanov2017variational}. \citet{stolcke1994bayesian} took a Bayesian approach to learning the structure of FSAs for modeling natural language by using the posterior probability of the model itself to balance goodness-of-fit criteria with model simplicity, thus encouraging simpler models.

Approaches which promote sparsity have a long history throughout machine learning and NLP. Recent approaches include sparseMAP \cite{sparsemap}, which allows for sparse structured inference, and sparsemax \cite{sparsemax}, which produces sparse attention mechanisms.


